A Massively Parallel Associative Memory Based on Sparse Neural Networks

Associative memories store content in such a way that the content can be later retrieved by presenting the memory with a small portion of the content, rather than presenting the memory with an address as in more traditional memories. Associative memories are used as building blocks for algorithms within database engines, anomaly detection systems, compression algorithms, and face recognition systems. A classical example of an associative memory is the Hopfield neural network. Recently, Gripon and Berrou have introduced an alternative construction which builds on ideas from the theory of error correcting codes and which greatly outperforms the Hopfield network in capacity, diversity, and efficiency. In this paper we implement a variation of the Gripon-Berrou associative memory on a general purpose graphical processing unit (GPU). The work of Gripon and Berrou proposes two retrieval rules, sum-of-sum and sum-of-max. The sum-of-sum rule uses only matrix-vector multiplication and is easily implemented on the GPU. The sum-of-max rule is much less straightforward to implement because it involves non-linear operations. However, the sum-of-max rule gives significantly better retrieval error rates. We propose a hybrid rule tailored for implementation on a GPU which achieves a 880-fold speedup without sacrificing any accuracy.

==> biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in]{photo/zhe.jpg}}]{Zhe Yao}
received his bachelor's degree in Telecommunication, in 2005, from Nanjing University of Posts and Telecommunications, Jiangsu, China.
He had been working in industry as both a Software Engineer and a System Engineer before resuming his academic education in Beijing University of Posts and Telecommunications, Beijing, China, where, in 2009, he obtained his master's degree in Communication and Information Systems.

Since 2009, he has been a Ph.D.\ student at Electrical and Computer Engineering Department, McGill University, Montr\'{e}al, QC, Canada, where he is currently a Ph.D.\ candidate.

His research interests involve machine learning, optimization, and parallel computing.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in]{photo/nophoto.jpg}}]{Vincent Gripon}
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in]{photo/mike.jpg}}]{Michael Rabbat} (S'02--M'12) received the B.Sc.~degree from the University of Illinois, Urbana-Champaign, in 2001, the M.Sc.~degree from Rice University, Houston, TX, in 2003, and the Ph.D.~degree from the University of Wisconsin, Madison, in 2006, all in electrical engineering.

He is currently an Assistant Professor at McGill University, Montr\'{e}al, QC, Canada. He was a Visiting Researcher at Applied Signal Technology, Inc., during the summer of 2003. His research interests include distributed information processing, network monitoring, and network inference. He is currently an Associate Editor for the \textit{ACM Transactions on Sensor Networks} and for \textit{IEEE Signal Processing Letters}.

Dr.~Rabbat received the Best Paper Award (Signal Processing and Information Theory Track) at the 2010 IEEE Conference on Distributed Computing in Sensor Systems, Outstanding Student Paper Honorable Mention at the 2006 Conference on Neural Information Processing Systems, and the Best Student Paper Award at the 2004 ACM/IEEE Conference on Information Processing in Sensor Networks.
\end{IEEEbiography}




==> emulate.tex <==
\section{Emulating \som{} with \sos{}\label{sec:emulate}}
Since \sos{} runs orders of magnitude faster, emulating \som{} using \sos{} seems to be another sensible choice.
We can follow the template of Algorithm \ref{alg:sumofsum} in Section \ref{sec:acceleration}.
The only necessary change is to convert the network matrix $W$ into a new weighted matrix $\Omega$ such that
\begin{equation}
	\forall i, j=1,2,\cdots,n\quad \Omega_{ij} = \begin{cases}
	0, &\mbox{if }w_{ij} = 0\\
	w_{ij}\theta^{\lfloor\frac{j-1}{L}\rfloor}, &\mbox{otherwise}
	\end{cases},\label{eq:emulate}
\end{equation}
where $\theta$ is a predefined basis parameter, which plays the role of carriers as in communications.
Instead of $WV^t$, we apply $\Omega V^t$.
The idea is to modulate signals from different clusters onto different exponential terms or carriers, and enjoy the speed of the matrix multiplication simultaneously.

For a given message $v^t$, $\Omega v^t$ generates a vector $u^t$ with all the signal information aggregated, which can be then used to determine the score function $s^t$.
The same as \sos{}, in each cluster, the neurons with the largest score value $s_i^t$, will stay activated to form $v^{t+1}$.
And the procedure repeats.

The final missing piece is how to obtain $s_i^t$ from $u_i^t$.
According to Equation \eqref{eq:emulate},
\begin{equation}
u_i^t=\sum_{j=1}^{n}{\Omega_{ij}v_j^t}=\sum_{c=1}^{C}{a_c\theta^{c-1}},
\end{equation}
where $a_c$, ranging from 0 to $L$, is the number of signals received from cluster $c$.
To investigate the contribution from cluster 1, we test if $a_1\neq 0$ by checking $u_i^t\mod{\theta}$.
Whenever true, it means neuron($i$) receives signals from cluster 1, and $s_i^t = s_i^t+1$.
This particular step regulates if multiple signals are received from the same cluster.
After testing $a_1$, setting $u_i^t=\lfloor\frac{u_i^t}{\theta}\rfloor$, we are ready to proceed $a_2$.

This attempt works flawlessly in theory, the only concern is the consequent network size because we only have fixed precision hardware.
We notice the exponential operations on the elements of $\Omega$, which makes $u_i^t$ a huge quantity.
In order to decouple the signals from different clusters completely, a conservative value is $\theta=L+1$.
The worst case happens when a neuron has connections to all the neurons (approximately, since no neuron could connect to the ones in the same cluster), which means we need some variable capable of holding the value $u_i^t=\sum_{c=1}^{C}{L(L+1)^{c-1}}=(L+1)^C-1$.
The smaller experiment setting in Section \ref{sec:experiment} has $C=8, L=128$, requiring $\log_2{(129^8-1)} \approx 56\mbox{ bits}$, which is already about the hardware precision limit, constraining the network size.
The easiest case is when exactly one signal comes from each cluster, which gives us the lower bound of 49 bits (the saved 7 bits correspond to the number of signals per cluster from previously $L=128$ down to 1), still despondent though.

In practice, other choices of $\theta\neq L+1$ can also be applied instead, e.g., if we tolerate some coupling between different clusters, a much smaller $\theta$ is able to postpone approaching to the hardware limit as the network scales up, without sacrificing too much retrieval rate.
In our experiment, we manage to apply $\theta=4$ to our larger scenario where $C=16$, $L=512$, 50000 messages to memorize and 30000 to test.
Although the number of iterations required is much higher than \som{} or even diverges, this emulation approach perfectly recovers the messages with half of the clusters erased, and runs much faster than \som{}.
However, when the problem becomes harder, e.g., the network gets saturated or the number of missing clusters increases, the performance degenerates.

